Multimodal Approach for Video Surveillance Indexing and Retrieval

In this paper, we present an overview of a multimodal system to indexing and searching video sequence by the content that has been developed within the REGIMVid project. A large part of our system has been developed as part of TRECVideo evaluation. The MAVSIR platform provides High-level feature extraction from audio-visual content and concept/event-based video retrieval. We illustrate the architecture of the system as well as provide an overview of the descriptors supported to date. Then we demonstrate the usefulness of the toolbox in the context of feature extraction, concepts/events learning and retrieval in large collections of video surveillance dataset. The results are encouraging as we are able to get good results on several event categories, while for all events we have gained valuable insights and experience.

==> files/abstract.tex <==
\thispagestyle{empty}

\noindent
{\bf\normalsize ABSTRACT}\newline
{In this paper, we present an overview of a new approach to indexing and search the video sequence by the content that has been developed within the REGIMVid project.   A large part of our system has been developed as part of TRECVID'2008 evaluation.
The platform termed REGIMVidToolbox provides Hight-level
feature extraction from audio-visual content and video search. Our subsystem
is based on the MPEG-7 eXperimental Model (XM),
with extensions to provide descriptor extraction from shaped image segments. Thereby, it supports local descriptors reflecting real image content. We describe the architecture
of the toolbox as well as providing an overview of the descriptors supported to date. We also briefly describe the search task. We then demonstrate the usefulness of the toolbox in the context of feature extraction, objects learning and retrieval in large collections of video surveillance dataset.}
\vspace{2ex}
   
\noindent
{\bf\normalsize KEY WORDS}\newline

{Feature fusion, Classifier fusion, Optical Flow, Active Contour, Support Vector Machines.}

==> files/ack.tex <==
\section*{Acknowledgements}


==> files/head.tex <==
\date{}
\title{High-level Features Extraction for Video Surveillance Indexing and Search}

\author{
Ali Wali ,Adel M. Alimi\\
Research Group on Intelligent Machines (REGIM)\\
University of Sfax\\
ENIS, BP 1173, Sfax 3038, Tunisia\\
email:{[ali.wali,adel.alim]@ieee.org} \\
}

\maketitle

